Unsupervised Parsing by Searching for Frequent Word Sequences among Sentences with Equivalent Predicate-Argument Structures

Unsupervised constituency parsing focuses on identifying word sequences that form a syntactic unit (i.e., constituents) in target sentences. Linguists identify the constituent by evaluating a set of Predicate-Argument Structure (PAS) equivalent sentences where we find the constituent appears more frequently than non-constituents (i.e., the constituent corresponds to a frequent word sequence within the sentence set). However, such frequency information is unavailable in previous parsing methods that identify the constituent by observing sentences with diverse PAS. In this study, we empirically show that constituents correspond to frequent word sequences in the PAS-equivalent sentence set. We propose a frequency-based parser span-overlap that (1) computes the span-overlap score as the word sequence's frequency in the PAS-equivalent sentence set and (2) identifies the constituent structure by finding a constituent tree with the maximum span-overlap score. The parser achieves state-of-the-art level parsing accuracy, outperforming existing unsupervised parsers in eight out of ten languages. Additionally, we discover a multilingual phenomenon: participant-denoting constituents tend to have higher span-overlap scores than equal-length event-denoting constituents, meaning that the former tend to appear more frequently in the PAS-equivalent sentence set than the latter. The phenomenon indicates a statistical difference between the two constituent types, laying the foundation for future labeled unsupervised parsing research.

==> acl_instruction.tex <==
\section{Introduction}

These instructions are for authors submitting papers to *ACL conferences using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} and this document contains additional instructions for the \LaTeX{} style files.

The templates include the \LaTeX{} source of this document (\texttt{acl.tex}),
the \LaTeX{} style file used to format it (\texttt{acl.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
  \begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
  \begin{verbatim}
\usepackage[review]{acl}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
  \begin{verbatim}
\usepackage{acl}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
  \begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
  \begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
  \centering
  \begin{tabular}{lc}
    \hline
    \textbf{Command} & \textbf{Output} \\
    \hline
    \verb|{\"a}|     & {\"a}           \\
    \verb|{\^e}|     & {\^e}           \\
    \verb|{\`i}|     & {\`i}           \\
    \verb|{\.I}|     & {\.I}           \\
    \verb|{\o}|      & {\o}            \\
    \verb|{\'u}|     & {\'u}           \\
    \verb|{\aa}|     & {\aa}           \\\hline
  \end{tabular}
  \begin{tabular}{lc}
    \hline
    \textbf{Command} & \textbf{Output} \\
    \hline
    \verb|{\c c}|    & {\c c}          \\
    \verb|{\u g}|    & {\u g}          \\
    \verb|{\l}|      & {\l}            \\
    \verb|{\~n}|     & {\~n}           \\
    \verb|{\H o}|    & {\H o}          \\
    \verb|{\v r}|    & {\v r}          \\
    \verb|{\ss}|     & {\ss}           \\
    \hline
  \end{tabular}
  \caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
  \label{tab:accents}
\end{table}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation:
\begin{quote}
  \tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
  \centering
  \begin{tabular}{lll}
    \hline
    \textbf{Output}           & \textbf{natbib command} & \textbf{ACL only command} \\
    \hline
    \citep{Gusfield:97}       & \verb|\citep|           &                           \\
    \citealp{Gusfield:97}     & \verb|\citealp|         &                           \\
    \citet{Gusfield:97}       & \verb|\citet|           &                           \\
    \citeyearpar{Gusfield:97} & \verb|\citeyearpar|     &                           \\
    \citeposs{Gusfield:97}    &                         & \verb|\citeposs|          \\
    \hline
  \end{tabular}
  \caption{\label{citation-guide}
    Citation commands supported by the style file.
    The style is based on the natbib package and supports all natbib citation commands.
    It also supports commands defined in previous ACL style files for compatibility.
  }
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

A possessive citation can be made with the command \verb|\citeposs|.
This is not a standard natbib command, so it is generally not compatible
with other style files.

\subsection{References}

\nocite{Ando2005,andrew2007scalable,rasooli-tetrault-2015}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
  \begin{verbatim}
\bibliography{custom}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
  \begin{verbatim}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya,
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu,
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan,
NAACL 2017 by Margaret Mitchell,
ACL 2012 by Maggie Li and Michael White,
ACL 2010 by Jing-Shin Chang and Philipp Koehn,
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui,
ACL 2005 by Hwee Tou Ng and Kemal Oflazer,
ACL 2002 by Eugene Charniak and Dekang Lin,
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

==> contents/fig-tbl-code/mean-skewness-perlang.tex <==

\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
        \hline
        Event       & English & Chinese & German & French & Hungarian & Swedish & Polish & Basque & Hebrew & Korean \\ \hline
        S           & 0.31    & -       & 0.21   & 0.19   & -         & 0.40    & 0.34   & 0.27   & 0.07   & -      \\ \hline
        VP          & 0.33    & 0.31    & 0.51   & 0.44   & -         & 0.60    & 0.37   & -      & 0.12   & 0.25   \\ \hline
        IP          & -       & 0.23    & -      & -      & -         & -       & -      & -      & -      & -      \\ \hline
        CP          & -       & 0.36    & -      & -      & 0.09      & -       & -      & -      & -      & -      \\ \hline
        Average     & 0.32    & 0.30    & 0.36   & 0.31   & 0.09      & 0.50    & 0.36   & 0.36   & 0.09   & 0.25   \\ \hline\hline
        Participant & English & Chinese & German & French & Hungarian & Swedish & Polish & Basque & Hebrew & Korean \\ \hline
        NP          & 0.68    & 0.46    & 0.76   & 0.57   & 0.44      & 0.73    & 0.70   & 0.55   & 0.31   & 0.43   \\ \hline
        PP          & 0.63    & 0.39    & 0.76   & 0.57   & 0.33      & 0.77    & -      & 0.52   & 0.21   & -      \\ \hline
        AP          & -       & -       & 0.73   & 0.56   & -         & 0.82    & -      & -      & -      & -      \\ \hline
        QP          & 0.77    & 0.49    & -      & -      & -         & -       & -      & -      & -      & -      \\ \hline
        Average     & 0.69    & 0.44    & 0.75   & 0.56   & 0.38      & 0.77    & 0.70   & 0.53   & 0.26   & 0.43   \\ \hline
    \end{tabular}
    \caption{Mean span-overlap scores for the event-denoting and the participant-denoting constituents. - indicates there is no annotation in the dataset for the corresponding phrase type. The Average entry shows the mean span-overlap scores averaged within the event-denoting and the participant-denoting constituents. }
    \label{tbl:mean-8-constituents}
\end{table*}

\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
        \hline
        Event       & English & Chinese & German & French & Hungarian & Swedish & Polish & Basque & Hebrew & Korean \\ \hline
        S           & 0.35    & -       & 1.13   & 1.12   & -         & 0.39    & 0.26   & 0.79   & 2.48   & -      \\ \hline
        VP          & 0.26    & 0.59    & -0.09  & 0.00   & -         & -0.28   & 0.15   & -      & 1.56   & 0.91   \\ \hline
        IP          & -       & 1.02    & -      & -      & -         & -       & -      & -      & -      & -      \\ \hline
        CP          & -       & 0.41    & -      & -      & 2.14      & -       & -      & -      & -      & -      \\ \hline
        Average     & 0.30    & 0.67    & 0.52   & 0.56   & 2.14      & 0.05    & 0.20   & 0.34   & 2.02   & 0.91   \\ \hline\hline
        Participant & English & Chinese & German & French & Hungarian & Swedish & Polish & Basque & Hebrew & Korean \\ \hline
        NP          & -0.93   & 0.06    & -1.34  & -0.45  & 0.20      & -0.94   & -0.99  & -0.38  & 0.63   & 0.13   \\ \hline
        PP          & -0.68   & 0.29    & -1.23  & -0.46  & -         & -1.02   & -      & -0.25  & 1.09   & -      \\ \hline
        AP          & -0.68   & -       & -1.23  & -0.46  & 0.47      & -1.46   & -      & -      & -      & -      \\ \hline
        QP          & -1.24   & 0.04    & -      & -      & -         & -       & -      & -      & -      & -      \\ \hline
        Average     & -0.95   & 0.13    & -1.26  & -0.45  & 0.33      & -1.14   & -0.99  & -0.315 & 0.86   & 0.13   \\ \hline
    \end{tabular}
    \caption{Skewness values for the event-denoting and the participant-denoting constituents. - indicates there is no annotation in the dataset for the corresponding phrase type. The Average entry shows the mean span-overlap scores averaged within the event-denoting and the participant-denoting constituents.}
    \label{tbl:skewness-8-constituents}
\end{table*}


==> contents/fig-tbl-code/score-spanlength-perlang-1.tex <==

\begin{figure*}[!ht]
    \centering
    % \begin{subfigure}[b]{0.24\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figs/english_dev.png}
    %     % \vspace{-0.6cm}
    %     \caption{English}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.24\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figs/chinese_dev.png}
    %     % \vspace{-0.6cm}
    %     \caption{Chinese}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/german_dev.png}
        % \vspace{-0.6cm}
        \caption{German}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/french_dev.png}
        % \vspace{-0.6cm}
        \caption{French}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/hungarian_dev.png}
        % \vspace{-0.6cm}
        \caption{Hungarian}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/swedish_dev.png}
        % \vspace{-0.6cm}
        \caption{Swedish}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/polish_dev.png}
        % \vspace{-0.6cm}
        \caption{Polish}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/basque_dev.png}
        % \vspace{-0.6cm}
        \caption{Basque}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/hebrew_dev.png}
        % \vspace{-0.6cm}
        \caption{Hebrew}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/korean_dev.png}
        % \vspace{-0.6cm}
        \caption{Korean}
    \end{subfigure}
    \hfill
    % \vspace{-0.3cm}
    \caption{Mean and skewness values of span-overlap scores. The values are measured over development sets and are grouped by their sequence lengths. }
    % \vspace{-0.5cm}
    \label{fig:mean'nskewness_by_spanlen}
\end{figure*}




% \begin{figure}[h]
%     \centering
%     \begin{subfigure}[b]{0.22\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/english_dev.png}
%         % \vspace{-0.6cm}
%         \caption{English}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{0.22\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/chinese_dev.png}
%         % \vspace{-0.6cm}
%         \caption{Chinese}
%     \end{subfigure}
%     \hfill
%     % \vspace{-0.3cm}
%     \caption{Mean and skewness values of span-overlap scores. The values are measured over development sets and are grouped by their sequence lengths. }
%     % \vspace{-0.5cm}
%     \label{fig:mean'nskewness_by_spanlen}
% \end{figure}

==> contents/fig-tbl-code/score-spanlength-perlang_copy.tex <==

% \begin{figure*}[!ht]
%     \centering
%     \begin{subfigure}[b]{0.19\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/english_dev.png}
%         % \vspace{-0.6cm}
%         \caption{English}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{0.19\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/chinese_dev.png}
%         % \vspace{-0.6cm}
%         \caption{Chinese}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.19\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/german_dev.png}
%         % \vspace{-0.6cm}
%         \caption{German}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{0.19\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/french_dev.png}
%         % \vspace{-0.6cm}
%         \caption{French}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.19\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/hungarian_dev.png}
%         % \vspace{-0.6cm}
%         \caption{Hungarian}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{0.19\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/swedish_dev.png}
%         % \vspace{-0.6cm}
%         \caption{Swedish}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.19\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/polish_dev.png}
%         % \vspace{-0.6cm}
%         \caption{Polish}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{0.19\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/basque_dev.png}
%         % \vspace{-0.6cm}
%         \caption{Basque}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.19\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/hebrew_dev.png}
%         % \vspace{-0.6cm}
%         \caption{Hebrew}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{0.19\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/korean_dev.png}
%         % \vspace{-0.6cm}
%         \caption{Korean}
%     \end{subfigure}
%     \hfill
%     % \vspace{-0.3cm}
%     \caption{Mean and skewness values of span-overlap scores. The values are measured over development sets and are grouped by their sequence lengths. }
%     % \vspace{-0.5cm}
%     \label{fig:mean'nskewness_by_spanlen}
% \end{figure*}




\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/english_dev.png}
        % \vspace{-0.6cm}
        \caption{English}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/chinese_dev.png}
        % \vspace{-0.6cm}
        \caption{Chinese}
    \end{subfigure}
    \hfill
    % \vspace{-0.3cm}
    \caption{Mean and skewness values of span-overlap scores. The values are measured over development sets and are grouped by their sequence lengths. }
    % \vspace{-0.5cm}
    \label{fig:mean'nskewness_by_spanlen}
\end{figure}

==> contents/old.2406/abstract.v3.tex <==
\begin{abstract}
    Unsupervised constituency parsing is about identifying word sequences that form a syntactic unit (i.e., constituents) in any target sentences.
    Linguists identify the constituent by evaluating a set of Predicate-Argument Structure (PAS) equivalent sentences where we find the constituent corresponds to frequent word sequences.
    However, such frequency information is unavailable to previous parsing methods which identify the constituent by observing sentences with diverse PAS.
    In this study, we empirically show that \textbf{constituents correspond to frequent word sequences in the PAS-equivalent sentence set}.
    We propose a frequency-based method \emph{span-overlap}, applying the frequency information to computational unsupervised parsing for the first time.
    The span-overlap parser achieves state-of-the-art level parsing accuracy, outperforming existing parsers in eight out of ten languages.
    Further analysis shows that the span-overlap parser effectively discriminates between constituents and non-constituents.
    The result highlights the utility of the frequency information.
    Additionally, we discover a multilingual phenomenon: \textbf{participant-denoting constituents are more frequent than equal-length event-denoting constituents in the PAS-equivalent sentence set}.
    The phenomenon indicates a behavioral difference between the two constituent types, laying the foundation for future labeled unsupervised parsing.


    
\end{abstract}


% The span-overlap method (1) generates a PAS-equivalent sentence set by instructing a Large Language Model with PAS-preserving instructions, and (2) measures the word sequence frequency in the generated sentence set.
%  the word sequence pattern that PAS-equivalent sentences reveal.
% linguists identify the constituent by evaluating whether the word sequence forms a string unit in a set of sentences whose Predicate-Argument Structures (PAS) are equivalent to that of the target sentence.
% Statistically, a string unit is more frequent than random strings in the PAS-equivalent sentence set, forming a word sequence pattern.
% However, previous parsing research identifies the constituent using sentences with diverse PAS, overlooking the word sequence pattern that PAS-equivalent sentences reveal.




% Parsing experiments show that the span-overlap parser outperforms state-of-the-art parsers in eight out of ten languages.
    % Further discrimination analysis confirms that the span-overlap method non-trivially separates constituents from non-constituents.
    % This result highlights the utility of the word sequence pattern.
    % Additionally, we discover a multilingual phenomenon: \textbf{participant-denoting constituents are more frequent than event-denoting constituents}.
    % The phenomenon indicates a behavioral difference between the two constituent types, laying the foundation for future labeled unsupervised parsing.




    % a set of Predicate-Argument Structure (PAS) equivalent sentences where the constituent is statistically more frequent than non-constituents.
    % However, 


    % evaluating whether a word sequence is statistically more frequent than random word sequences in a set of sentences that have Predicate-Argument Structures (PAS) equivalent to the PAS of the target sentence.
    % However, previous parsing research does not utilize PAS-equivalent sentences, overlooking the constituent-related information that the word sequence frequency provides.
    % In this study, we empirically verify a hypothesis, \textbf{constituents correspond to frequent word sequences in the PAS-equivalent sentence set}.
    % We propose a frequency-based method \emph{span-overlap} to exploit the word sequence frequency information.
    % Parsing experiments show that the span-overlap parser outperforms state-of-the-art parsers in eight out of ten languages, highlighting the utility of the frequency information.
    % Analysis of constituent frequencies indicates that the span-overlap parser can effectively distinguish between constituents and non-constituents.
    % Analysis by constituent types reveals a multilingual phenomenon: \textbf{participant-denoting constituents are more frequent than event-denoting constituents}, indicating a behavioral difference between the two types of constituents.
    % Ablation analysis indicates the necessity of combining multiple PAS-preserving instructions to effectively reveal the constituent structure.

==> contents/old.2406/experiments.tex <==
\section{Experiment}
\label{sec:experiment}
\input{contents/fig-tbl-code/f1-spmrl}
\subsection{Experimental Settings}
We conduct experiments in 10 languages, namely English (Penn Treebank (PTB) \cite{Treebank-3}), Chinese (Penn Chinese Treebank 5.1 (CTB) \cite{CTB5.1}\footnote{The PTB and CTB datasets are available under the \texttt{LDC User Agreement for Non-Members} license.}), German, French, Hungarian, Swedish, Polish, Basque, Hebrew, and Korean (SPMRL \cite{seddah-etal-2013-overview}).
We apply the same training/development/testing split as \citet{li-lu-2023-contextual}. %for the PTB and CTB dataset \footnote{The datasets are available under the \texttt{LDC User Agreement for Non-Members} license}, and the official split for the SPMRL dataset, following previous evaluation settings \cite{li-lu-2023-contextual}.
We use the development section for analysis and the testing section for comparison with existing unsupervised parsers.
As per previous research \cite{DBLP:conf/iclr/ShenLHC18, kim-etal-2019-compound}, we evaluate the parsing accuracy using the unlabelled sentence-F1 (SF1) score on sentences of length $\geq$ 2.
We drop punctuation (e.g., comma and period) and trivial spans (i.e., span of size 1 and sentence level span) when computing the SF1 score.

We generate PAS-equivalent sentences using an instruction-following LLM \texttt{GPT-3.5-turbo-0125}.
We apply English instructions for all languages but add a specific directive asking the LLM to generate native samples in non-English languages.
We manually examined 100 samples in English and Chinese, and found most samples have PAS identical or similar to the target sentence.\footnote{More details in Appendix~\ref{sec:appendix-samplequality}}
% We refer the readers to Appendix~\ref{sec:appendix-samplequality} for more details.
We apply the snowball-stemmer\footnote{Available as a part of the NLTK package.} for English, French, German, Basque, Hungarian, and Swedish, and the stempel-stemmer\footnote{Available as a part of \href{https://www.egothor.org/product/egothor2/index.html}{the egothor project.}} for Polish.
We skip the stemming process for Chinese, Korean, and Hebrew.
Chinese words do not take inflections.
Hebrew and Korean do not have a readily available stemmer.
We normalize contractions only in English and French, because of the common use of contractions in these languages.
% the contraction rules in the two languages are simple and the contraction affects a large portion of the dataset.
While not implementing the full normalization may harm the parsing accuracy in many languages, the span-overlap parser achieves state-of-the-art level performance without the normalization in those languages.

We analyze the frequency for two types of constituents: participant-denoting and event-denoting constituents.
The objective is to identify how the language model behaves when generating constituents of different characteristics.
We refer to a constituent as participant-denoting when it denotes a participant in the PAS.
Likewise, we refer to a constituent as event-denoting when it denotes an event in the PAS.
For example, Noun Phrases (NP) and Prepositional Phrases (PP) are common participant-denoting constituents, whereas Verb Phrases (VP) and Inflectional Phrases (IP) are common event-denoting constituents.
We compare the frequency for phrase types with more than twenty occurrences.
We normalize the phrase type annotation for three languages (French, Polish, and Basque) whose annotation does not align with the PTB's annotation.
In French, we merge the \texttt{Srel}, \texttt{Sint}, and \texttt{Ssub} phrases into S, and the \texttt{VPpart} and \texttt{VPinf} into VP.
In Polish, we treat the \texttt{zdanie} phrase as S, the \texttt{fwe} as VP, and the \texttt{fno} as NP \cite{wolinski-etal-2018-new}.
In Basque, we treat the \texttt{SN} phrase as NP and the \texttt{SP} phrase as PP \cite{DBLP:journals/pdln/SanchezFAA08}.


\subsection{Comparison with the State-of-the-Art}

\begin{table}[t]
    \small
    \centering
    % \vspace{-0.2cm}
    \adjustbox{width=0.8\columnwidth}{
        \begin{tabular}{|l|ll|}
            \hline       & English              & Chinese       \\\hline
            GPT 3.5     & 36.2       & 5.1    \\\hline
            N-PCFG\dag   & 50.8      (50.8)     & 29.5  (34.7)  \\
            C-PCFG\dag   & 55.2  (52.6)         & 39.8   (37.3) \\
            TN-PCFG\dag  & \textbf{57.7} (51.2) & 39.2 (39.3)   \\\hline
            MLM-IP\ddag  & 49.0 (46.4)          & -   (37.8)    \\
            Span Overlap & 52.9                & \textbf{48.7} \\\hline
        \end{tabular}}
    \caption{SF1 score on the English (PTB) and the Chinese (CTB) test set. The best results are highlighted in bold. \dag: results from \cite{yang-etal-2021-pcfgs}; \ddag: results from \cite{li-lu-2023-contextual}; -: result not reported. Numbers in parentheses () are our reproduction with the released code and data. Reproduction results for the PCFG-based methods are the average of four independent runs.}
    \label{tbl:ptbnctb-comprison}
    % \vspace{-0.5cm}
\end{table}


Table~\ref{tbl:spmrl-comparison} and Table~\ref{tbl:ptbnctb-comprison} showcase the effectiveness and applicability of the frequency information revealed in the PAS-equivalent sentence set.
The two tables compare the span-overlap parser with three PCFG-based parsers (N-PCFG, C-PCFG \cite{kim-etal-2019-compound}, and TN-PCFG \cite{yang-etal-2021-pcfgs}) and the latest language model-based parser (MLM-IP \cite{li-lu-2023-contextual}).
We also include a GPT-3.5 parser that predicts PTB style parse tree in its serialized form (e.g., ``(S (NP (DT The) (NN value)) (VP (VBD was) (VP (VBN disclosed))))'').
We drop trivial and duplicate spans when computing the unlabelled SF1 score for the GPT-3.5 parser. 



The span-overlap parser represents a significant improvement over previous unsupervised parsers, outperforming the best baseline parser in eight out of ten languages.
The span-overlap parser outperforms the MLM-IP parser by 3.99 SF1, 10.9 SF1, and 4.32 mean SF1 scores in the English PTB, the Chinese CTB, and the multilingual SPMRL dataset, respectively.
It respectively outperforms the best grammar-based parser (TN-PCFG) by 9.5 SF1 and 9.31 mean SF1 scores in the Chinese CTB and the multilingual SPMRL dataset, but underperforms the TN-PCFG parser by 4.7 SF1 score in the English PTB dataset.
The high parsing accuracy establishes the span-overlap parser as a simple but competitive multilingual unsupervised constituent parser.

The strong parsing performance is not solely due to the application of the \texttt{GPT-3.5} model.
As shown in the table, the GPT-3.5 parser is the worst-performing baseline parser in the PTB, CTB, and SPMRL dataset, achieving 36.2 SF1 in the PTB, 0.1 SF1 in the CTB, and 23.25 mean SF1 score in the SPMRL dataset.
The low parsing accuracy indicates that the GPT-3.5 model can only recover a small portion of constituent structure.
In contrast, the proposed span-overlap parser uncovers significantly more constituent structures, outperforming the GPT-3.5 parser by 16.7 SF1 in the PTB, by 43.6 SF1 in the CTB, and by 26.86 mean SF1 score in the SPMRL dataset.






% The GPT-3.5 parser that directly outputs binary trees performs poorly in a dataset-level, with the worst accuracy amongst all baseline parsers.
% This is because the GPT-3.5 can only parse a small portion of the dataset.
% In our experiment, the proportion of sentences successfully parsed by the GPT-3.5 parser ranges from 10\% to 30\%.
% In contrast, the span-overlap parser always yields a valid parse tree for any given sentences, ensuring a high dataset-level accuracy.
% The span-overlap parser outperforms the GPT-3.5 parser in all languages when using both the dataset-level SF1 score and the SF1 score for sentences that the GPT-3.5 parser successfully parsed.
% The significant improvement in parsing accuracy illustrates that the span-overlap parser is more than a mere application of the \texttt{GPT-3.5} model to unsupervised parsing.


% Even when comparing using the SF1 score for sentences that the \texttt{GPT-3.5} parser successfully parsed


% the large gap between the SF1 score for all sentences and the score for successfully parsed sentences.





% Compared to the MLM-IP parser, the span-overlap parser outperforms the MLM-IP parser by 3.99 and 10.9 SF1 scores in the English PTB dataset and the Chinese CTB dataset, respectively.
% The span-overlap parser obtains a 4.32 mean SF1 score improvement in the multilingual SPMRL dataset.
% Compared to the grammar-based parsers, the span-overlap parser outperforms all grammar-based parsers in nine out of ten languages.
% The span-overlap parser improves the best grammar-based parser by 9.5 SF1 score in the CTB dataset and by 9.31 mean SF1 score in the SPMRL dataset.
% Compared to the \texttt{GPT-3.5} parser, the


% Table~\ref{tbl:ptbnctb-comprison} presents the comparison in English and Chinese.
% The span-overlap parser outperforms the MLM-IP parser by 3.99 and 10.9 SF1 scores in English and Chinese, respectively.
% The span-overlap parser outperforms all grammar-based parsers in Chinese by a margin of at least 8.9 SF1 score.
% In English, the span-overlap parser underperforms the C-PCFG and TN-PCFG parsers when using the reported accuracy but outperforms all grammar-based parsers when using our reproduced accuracy.
% Table~\ref{tbl:spmrl-comparison} presents the comparison in the other eight languages.
% The span-overlap parser outperforms the MLM-IP parser, the best baseline parser, by 4.32 mean SF1 score.
% The span-overlap parser performs significantly better or comparable to the MLM-IP parser in all languages except Hebrew.
% Hebrew is a morphologically rich language for which we have no readily available stemmer to remove morphological features.
% The rich morphological feature obstructs the word-matching process in the span-overlap method, which leads to an underestimation of the word sequence frequency.
% Other morphologically rich languages (e.g., Swedish) do not suffer from the lack of stemmer, enjoying a significantly better performance.
% Overall, the parsing result establishes the span-overlap parser as a simple but competitive multilingual unsupervised constituency parser.

% The span-overlap parser obliterates the \texttt{GPT-3.5} parser in terms of parsing accuracy.
% The \texttt{GPT-3.5} parser performs poorly at the corpus level, which agrees with \citet{DBLP:journals/corr/abs-2310-19462}'s result.
% The \texttt{GPT-3.5} parser has the worst accuracy amongst all baseline parsers, due to the large number of sentences that the \texttt{GPT-3.5} parser failed to parse.
% In our experiment, the \texttt{GPT-3.5} parser successfully parses around 10\% to 30\% of the sentences in the corpus, which explains the large gap between the SF1 score for all sentences and the score for successfully parsed sentences.
% Most of the successfully parsed sentences are short sentences.
% The span-overlap parser has higher accuracies than the \texttt{GPT-3.5} parser in all languages, even when only sentences successfully parsed by the \texttt{GPT-3.5} parser are considered.
% %  compared using the SF1 score for successfully parsed sentences.
% % outperforms the \texttt{GPT-3.5} parser in all languages when compared even using the SF1 score for successfully parsed sentences.
% The comparison is heavily in favor of the \texttt{GPT-3.5} parser because the SF1 score tends to be higher for short sentences.
% The higher accuracy of the span-overlap parser suggests that the span-overlap method recovers non-trivial constituent structures that the \texttt{GPT-3.5} model cannot recover.

\input{contents/fig-tbl-code/score-mean-distribution-english}
\input{contents/fig-tbl-code/score-spanlength-perlang}


\subsection{Participant-denoting Constituents are More Frequent than Equal-length Event-denoting Constituents}
In this section, we demonstrate a frequency difference between equal-length participant-denoting and event-denoting constituents within the set of PAS-equivalent sentences.
We observe the frequency difference through the span-overlap score which represents the word sequence frequency within the PAS-equivalent sentence set. 
We focus on four participants-related constituents (i.e., Noun Phrases (NP), Prepositional Phrases (PP), Adpositional Phrases (AP), and Quantifier Phrases (QP)) and four event-denoting constituents (i.e., Declarative Clauses (S), Verb Phrases (VP), Inflectional Phrases (IP), and Complementizer Phrases (CP)).
We also include the span-overlap score for random word sequences that have the same sequence length statistics as gold constituents (i.e., For each random sequence, there is a gold constituent having the same sequence length).

% In this section, we analyze the span-overlap score by phrase types.
% We observed a \emph{multilingual} phenomenon: \textbf{participant-denoting constituents tend to have higher span-overlap scores (i.e., more frequent) than event-denoting constituents}.
% We focus on four participants-related constituents (i.e., Noun Phrases (NP), Prepositional Phrases (PP), Adpositional Phrases (AP), and Quantifier Phrases (QP)) and four event-denoting constituents (i.e., Declarative Clauses (S), Verb Phrases (VP), Inflectional Phrases (IP), and Complementizer Phrases (CP)).
% We also include data points for \emph{random} word sequences with the same sequence length statistics as gold constituents (i.e., Each gold constituent has an equal-length random word sequence as its counterpart.).



We begin by observing the frequency difference in the English PTB dataset.
Figure~\ref{fig:mean_scores'ndistributions} shows the mean span-overlap score along with the score distribution for NP, PP, QP, S, and VP.
The AP, IP, and CP are not annotated in the PTB dataset and, therefore, cannot be shown in the figure.
The three participant-denoting constituents (i.e., NP, PP, and QP) have higher mean scores than the two event-denoting constituents (i.e., S and VP).
The distribution figure shows that most participant-denoting constituents have high scores whereas most event-denoting constituents do not.
We can characterize this feature using the skewness value of the score distribution \cite{Russo2020}.
A negative skewness value indicates more constituents with high scores than those with low scores.
In English, the participant-denoting constituents have a negative skewness value, whereas the event-denoting constituents have a positive skewness value.
Interestingly, the random word sequence has a similar mean score and skewness value to the event-denoting constituents.
The comparison indicates a statistical difference between the participant-denoting constituents and the event-denoting constituents.


% Interestingly, the mean frequency for the two event-denoting constituents is similar to that for the random word sequence.
% The picture becomes increasingly apparent in the score distribution figures.
% The span-overlap scores for the participant-denoting constituents concentrate around the maximum value, whereas the scores for the event-denoting constituents concentrate around the minimum value.
% We can characterize the score concentration with skewness \cite{Russo2020}.
% A negative skewness value indicates more constituents with high span-overlap scores than those with low scores.
% We conjecture that the participant-denoting constituents are more frequent than the event-denoting constituents in the PAS-equivalent sentence set.

Figure~\ref{fig:mean'nskewness_by_spanlen} confirms that the frequency difference is a multilingual phenomenon and is not mere a by-product of the frequency-length correlation.
As shown in the figure, short constituents tend to have higher scores than long constituents, prompting the question of whether the frequency difference is due to the length difference.
This is unlikely the case.
As illustrated in the figure, participant-denoting constituents are noticeably more frequent than equal-length event-denoting constituents over \emph{all sequence lengths}.
The skewness values for the participant-denoting constituents are lower than those for the event-denoting constituents.
This indicates that there are more participant-denoting constituents with high scores than those with low scores.
In other words, participant-denoting constituents are more frequent than equal-length event-denoting constituents.
We include the data for the other eight languages in Figure~\ref{fig:mean'nskewness_by_spanlen-appendix}, which shows the same trend across all languages evaluated.
However, there are some language-specific differences despite the general trend.
For example, the score gap between the two constituent types is very clear in English but not so much in Chinese.
The score of the event-denoting constituents in English is similar to the score of the random word sequences, whereas the score of the event-denoting constituents in Chinese is much higher than the score of the random word sequences.

This analysis highlights a statistical difference between equal-length participant-denoting constituents, event-denoting constituents, and random word sequences. 
The analysis sheds lights on future unsupervised parsing with phrase labels.

% This analysis, on the one hand, showcases the effectiveness of the frequency information in separating constituents and non-constituents.
% On the other hand, it highlights the statistical difference between participant-denoting constituents, event-denoting constituents, and random sequences.





% Figure~\ref{fig:mean'nskewness_by_spanlen} confirms our conjecture, presenting the mean scores and skewness values in ten languages.
% Starting with English, we have two observations:
% (1) the participant-denoting constituents tend to have higher mean scores and lower skewness values than the event-denoting constituents for all sequence lengths;
% A statistics gap is present between the two constituent types in most languages, confirming our conjecture.
% (2) the random word sequences have mean scores and skewness values similar to the event-denoting constituents for short sequence lengths.
% The statistics gap between the random sequences and event-denoting constituents gradually enlarges as the sequence length goes longer, indicating a fundamental difference between the random sequences and event-denoting constituents.
% We can make similar observations in other languages, with some degree of fluctuations.
% For example, the separation between the two constituent types in Chinese is less pronounced than in other languages.
% VP in French, an event-denoting constituent, is closer to participant-denoting constituents than to S, another event-denoting constituent.
% That being said, we can observe a general trend: the participant-denoting constituents have higher span-overlap scores than the event-denoting constituents.

% This analysis, on the one hand, indicates the effectiveness of the span-overlap score in separating constituents and non-constituents.
% On the other hand, the analysis highlights the statistical difference between participant-denoting constituents, event-denoting constituents, and random sequences.

\subsection{Span-overlap Score Distinguishes between Constituents and Non-constituents}
\input{contents/fig-tbl-code/proportion.tex}
\input{contents/fig-tbl-code/tbl-ablation}
This experiment provides a glimpse of the discriminating power of the span-overlap score.
We compare the span-overlap score with random scores in terms of whether the score can identify the constituent in a set of mutually incompatible word sequences.
The random score is uniformly sampled from [0, 1], the same range as the span-overlap score.
We measure the proportion of gold constituents to which the score assigns a strictly higher value than all incompatible non-constituents.
We refer to a non-constituent as incompatible with a gold constituent when the two sequences partially overlap (i.e., they cannot co-exist in the same tree).

Figure~\ref{fig:proportions} plots the proportion by word sequence lengths.
The span-overlap score distinguishes between constituents and non-constituents, identifying more constituents than the random score for all sequence lengths and in all languages.
In the European languages, the span-overlap parser reliably identifies around 50\% of constituents, regardless of the constituents' length.
The random parser, on the other hand, identifies around 40\% of short constituents but only around 10\% of long constituents.
The comparison highlights the effectiveness of the span-overlap score in identifying constituents, especially for long constituents.
However, Chinese and Korean seems to be an exception.
Whilst the span-overlap parser still identifies more constituents than the random parser, the proportion drops for long constituents. 
This is because the span-overlap parser could not find any long word sequences that appear in both the target sentence and the generated PAS-equivalent sentences.
The problem might be related to the sample quality problem that we will discuss in Section~\ref{sec:limitations}.
% Overall, the span-overlap score exhibits a strong discriminative power, although the quality of the PAS-equivalent sentences limits such power.



% In languages other than Chinese and Korean, the proportion for the span-overlap score maintains at a high level, indicating the span-overlap score's effectiveness in identifying constituents.
% The proportion in Chinese and Korean rapidly decreases so that the proportion is lower (Chinese) or similar to (Korean) the score for the random score.
% The problem might be related to the sample quality problem that we will discuss in Section~\ref{sec:limitations}.
% Overall, the span-overlap score exhibits a strong discriminative power, although the quality of the PAS-equivalent sentences limits such power.



\subsection{Ablation of PAS-Preserving Instructions}


Table~\ref{tbl:ablation} showcases the benefit of aggregating multiple PAS-preserving instructions.
The table compares the span-overlap parser with only one instruction type and with all six instruction types.
Even with a single instruction type, the span-overlap parser outperforms the random, right-branching, and \texttt{GPT-3.5} parsers.
This result suggests that the span-overlap method uncovers non-trivial constituent structures.
The best parser with a single instruction type is always the one with the movement instruction.
The phenomenon suggests a fundamental role of movable constituents in identifying constituent structures.
Combining all instruction types sees significant improvements in parsing accuracy.
The average improvement is 3.09\% SF1 score between the parser with all instruction types and the best parser with a single instruction type.
This result indicates the benefit and necessity of aggregating multiple instructions in generating the PAS-equivalent sentence set.










==> contents/old.2406/introduction.v2.tex <==
\section{Introduction}

\begin{figure}[t]
    \centering
    \includesvg[inkscapelatex=false, width=0.8\columnwidth]{figs/figures-TargetnThematicEquivalentExamples.drawio.svg}
    \caption{A target sentence and a set of PAS-equivalent sentences. We highlight in bold constituents that are frequent in the PAS-equivalent sentence set.}
    \label{fig:thematic_equiv_example}
    % \vspace{-0.6cm}
\end{figure}

\newcommand\blfootnote[1]{
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

% /footnote{The code and data are available at \url{}}
\blfootnote{We release the code and data at \url{https://github.com/junjiechen-chris/ACL24-SpanOverlap}}
Unsupervised constituency parsing is about identifying the constituent structure for any target sentences.
The constituent structure consists of a set of syntactically self-contained word sequences, commonly known as constituents.
Those constituents also encode semantic units in the sentence's semantic structure \cite{Carnie2007-CARSAG, Fasold_Connor-Linton_2014}.
Among all possible word sequences that can arise in natural language, the constituent in one of the few word sequences that can describe the semantic unit.
% The constituents are one of the few word sequences that can describe the semantic unit.
As a result, we would have a higher chance of repeatedly observing the constituent than random word sequences given the semantic unit.
In other words, we can observe the constituent as a frequent word sequence in sentences that are semantically equivalent.
% In other words, the constituent would correspond to a frequent word sequence in the semantically equivalent sentence set.
We refer to the frequent word sequence as a \emph{word sequence pattern}.


% Those constituents often encompass semantic units in the target sentence's semantic structure \cite{Carnie2007-CARSAG, Fasold_Connor-Linton_2014}.
% The constituent is one of the few word sequences that describe the semantic unit.
% As a result, we would have a higher chance of repeatedly observing the constituent than random word sequences in a set of sentences that are semantically equivalent to the target sentence.
% In other words, the constituent would correspond to a frequent word sequence in the semantically equivalent sentence set.
% We refer to the frequent word sequence as a \emph{word sequence pattern}.

In this paper, we empirically show a hypothesis: \textbf{constituents correspond to frequent word sequences in the set of sentences with equivalent Predicate-Argument Structures (PAS)}.
PAS abstracts the sentence semantics as an event with three elements:  (1) predicates of the event; (2) participants of the event (i.e., arguments); (3) the semantic relationship between the predicates and arguments (i.e., thematic relations) \cite{palmer-etal-2005-proposition} (Figure~\ref{fig:thematic_equiv_example}).
We refer to two sentences as \emph{Predicate-Argument Structure (PAS) equivalent} when they have the same PAS elements.
Controlling the PAS provides a good approximation to controlling the semantic structure.
Figure~\ref{fig:thematic_equiv_example} exemplifies our hypothesis with a target sentence, ``John ate an apple this morning.''
Word sequences like ``an apple'' are constituents in the target sentence, whereas word sequences like ``John ate'' are non-constituents.
Compared to the non-constituent, the constituents occur more frequently in the target sentence's PAS-equivalent sentence set, manifesting itself as a word sequence pattern.
% Experiments demonstrates the effectiveness and the applicability of the frequency information.
% The 
% We also show the applicability and effectiveness of the frequency information in unsupervised parsing.


\begin{table}[t]
    \adjustbox{max width=1\columnwidth}{
        \centering
        % \small
        \begin{tabular}{|l|l|}
            \hline
            \multirow{4}{*}{Treebank           }   & Results were released after the market closed.      \\
             & Markets stopped trading in many securities. \\
             & Mr. Bandow is a Cato Institute fellow.      \\\hline
            \multirow{4}{*}{Constituency Test  } & It's an apple that John eats this morning.          \\
             & What John eats this morning is an apple.    \\
             & An apple, John eats this morning            \\\hline
        \end{tabular}
    }
    \caption{A comparison of data in Penn Treebank and data produced by constituency tests. The constituency test data are byproducts of testing the constituency of ``an apple''.}
    \label{tbl:treebank_vs_linguistics}
    % \vspace{-0.4cm}

\end{table}

However, such frequency information was not available to previous unsupervised parsing methods.
Those previous methods focused on uncovering the constituent structure by either inducing a complex grammar \cite{kim-etal-2019-compound, yang-etal-2021-pcfgs} or evaluating whether a word sequence can withstand syntactic transformations \cite{cao-etal-2020-unsupervised, wu-etal-2020-perturbed, li-lu-2023-contextual}.
Both methods operate upon sentences with diverse PAS, as shown in the upper half of Table~\ref{tbl:treebank_vs_linguistics}.
These sentences provide little information about the constituent structure, as evidenced by the low frequency of word sequences corresponding to constituents.
Linguistic researchers perform constituency tests (e.g., movement) \cite{Carnie2007-CARSAG} using handcrafted sentences with equivalent PAS, as shown in the lower half of Table~\ref{tbl:treebank_vs_linguistics}.
These PAS-equivalent sentences, as discussed above, provide significantly more information about the constituent structure, as evidenced by the high frequency of word sequences corresponding to constituents.
The gap in data characteristics motivates our research on unsupervised parsing using PAS-equivalent sentences.

We apply the hypothesis to unsupervised parsing and propose a frequency-based method, \emph{span-overlap}, to exploit the frequency information.
The span-overlap method uncovers constituents by identifying high frequency word sequences in PAS-equivalent sentences generated by a Large Language Model (LLM).
Parsing experiments confirm our hypothesis, highlighting the utility and applicability of the frequency information to unsupervised parsing.
The span-overlap parser obtains higher parsing accuracy than state-of-the-art unsupervised parsers in eight out of ten languages evaluated and by a large margin.
The span-overlap parser can effectively separate constituents from non-constituents, especially for long constituents.
In addition to the hypothesis, we discover a multilingual phenomenon:  \textbf{participant-denoting constituents are more frequent than equal-length event-denoting constituents in the PAS-equivalent sentence set}.
The phenomenon indicates a behavioral difference between the two constituent types, laying the foundation for future unsupervised parsing with labels.


% We propose a frequency-based method \emph{span-overlap}, applying the word sequence pattern to computational unsupervised parsing for the first time.
% Given a target sentence, the span-overlap method discovers the word sequence pattern in a set of PAS-equivalent sentences that are generated by a Large Language Model (LLM).
% Parsing experiments verify our hypothesis and highlight the utility and applicability of the word sequence pattern to unsupervised parsing.\footnote{Applying the PAS-equivalent sentences to grammar induction significantly improves the grammar's parsing performance. Please refer to Appendix~\ref{sec:appendix-gi_with_pas} for more details.}.
% Our span-overlap parser outperforms state-of-the-art unsupervised parsers in eight out of ten languages evaluated, usually by a large margin.
% Our method can separate significantly more constituents from non-constituents than a random baseline.
% In addition to the hypothesis, we discover a multilingual phenomenon:  \textbf{participant-denoting constituents are more frequent than event-denoting constituents}.
% The phenomenon indicates a behavioral difference between the two constituent types, laying the foundation for future unsupervised parsing with labels.




% %! contrast the difference in data characteristic
% Previous unsupervised parsing research focused on either inducing a complex grammar from a plain text corpus \cite{kim-etal-2019-compound, yang-etal-2021-pcfgs} or evaluating whether a word sequence is a constituent using language models \cite{cao-etal-2020-unsupervised, wu-etal-2020-perturbed, li-lu-2023-contextual}.
% Both methods operate upon sentences with diverse PAS (the upper half of Table~\ref{tbl:treebank_vs_linguistics}).
% These sentences provide little information about the constituent structure, as evidenced by the low frequency of word sequences corresponding to constituents.
% In linguistic studies, researchers perform constituency tests \cite{Carnie2007-CARSAG} using handcrafted sentences with equivalent PAS (the lower half of Table~\ref{tbl:treebank_vs_linguistics}).
% These sentences provide significantly more information about the constituent structure, as evidenced by the high frequency of word sequences corresponding to constituents.
% The gap in data characteristics motivates our research on unsupervised constituency parsing using PAS-equivalent sentences.


% In this study, we propose a frequency-based method \emph{span-overlap}.
% The span overlap method consists of two steps: (1) generates a PAS-equivalent sentence set for each target sentence; (2) measures the word sequence frequency in the generated sentence set.
% We generate the PAS-equivalent sentence set by instructing a Large Language Model (LLM) to perform PAS-preserving transformations.
% The generated sentence set provides constituent-related information that was only accessible through handcrafted PAS-equivalent sentences at a large scale.
% Parsing experiments show that the span-overlap parser outperforms state-of-the-art unsupervised parsers in eight out of ten languages, despite the simplicity of our method.
% An analysis of word sequence frequencies shows that the span-overlap method can distinguish between constituents and non-constituents.
% On one hand, this result verifies our hypothesis that constituents indeed correspond to frequent word sequences in the PAS-equivalent sentence set.
% On the other hand, the result indicates the effectiveness and applicability of the word sequence pattern for discovering the constituent structure 
% A close examination by constituent types reveals a \emph{multilingual} phenomenon: \textbf{participant-denoting constituents are more frequent than event-denoting constituents}.
% The phenomenon indicates a behavioral difference between the two types of constituents which encode frame semantics \cite{Fillmore2001FrameSF} at different levels.
% An ablation analysis suggests the necessity of combining multiple PAS-preserving transformations for comprehensively exposing the constituent structure.


==> contents/old/abstract.tex <==
% invariable?
\begin{abstract}
    Unsupervised constituency parsers recover a sentence's phrase structure without relying on structural annotation data.
    When analyzing for the phrase structure, linguists compare sentences with similar semantics to isolate syntactic factors to word-sequence patterns from semantic factors.
    However, current unsupervised constituency parsers derive the phrase structure using sentences where the word-sequence pattern can be attributed to both the syntactic and the semantic factors.
    In this paper, we explore the potential of semantic control in unsupervised constituency parsing.
    We control the sentence semantics through fixing the sentence's thematic relations.
    The thematic relations specify the relationship between an event and its participants.
    We hypothesize that constituents are frequent word-sequences among thematically equivalent sentences and devise a span-overlap score to measure the word-sequence frequency
    We sample the thematically equivalent sentences from large language models using 4 types of theme-preserving instructions.
    The resulting span-overlap score is discriminative of gold constituents and the resulting parser outperforms state-of-the-art unsupervised constituency parsers in a multilingual experiment.
    Analysis reveals that constituents denoting an event's participants are more cohesive units than constituents denoting the event, indicating a behavioral difference between the two types of constituents.
\end{abstract}


==> contents/old/abstract.v2.tex <==
% invariable?
\begin{abstract}
Unsupervised constituency parsing aims to identify a sentence's constituent structure without structural annotation data.
Linguists test for constituents by evaluating a set of sentences with equivalent Predicate-Argument Structures (PAS), where the constituent is a frequent word sequence.
However, current unsupervised parsers search for constituents using sentences with diverse PAS, missing out on the constituent-related word sequence pattern that is easily identifiable through the control of PAS.
In this study, we hypothesize that \textbf{constituents are frequent word sequences among sentences with equivalent predicate-argument structures}.
We propose a span-overlap score to measure the word sequence frequency among the PAS-equivalent sentences.
Experiments show that the span-overlap score is discriminative of constituents and non-constituents.
The resulting parsing model outperforms existing unsupervised parsers in multilingual evaluations, indicating the benefit of PAS controls.
Further analysis reveals a linguistically universal phenomenon: participant-denoting constituents are more frequent than event-denoting constituents, indicating a behavioral difference between the two types of constituents.
Ablation analysis shows that combining multiple PAS-preserving transformations is beneficial to comprehensively exposing the constituent structure.
\end{abstract}


==> contents/old/discussion.tex <==
\section{Discussion}
% <Connection with data augmentation>

% <poor perf. with soft score>

==> contents/old/introduction.tex <==
\section{Introduction}
Unsupervised constituency parsing aims to identify the phrase structure of natural language sentences.
A phrase structure consists of multiple constituents that are word sequences functioning as a single unit.
The phrase structure provides much information for Natural Langauge Processing (NLP) systems (e.g., machine translation \cite{eriguchi-etal-2019-incorporating} and semantic parsing \cite{das-etal-2014-frame, marcheggiani-titov-2020-graph}).
What underlies the syntax-assisted NLP system is the correlation between syntactic and semantic units, as illustrated in Figure~\ref{fig:thematic_equiv_def}
The three semantic units (i.e., \textit{John}, \textit{an apple}, and \textit{this morning}) are themselves syntactic units in the sentence's phrase structure.
Psychological studies also suggest a strong correlation between phrase structures and human semantic processing of language \cite{Nelson2017NeurophysiologicalDO}.
In this paper, we explore the possibility of uncovering phrase structures by controlling sentence semantics.


\begin{figure}[t]
    \centering
    \includesvg[inkscapelatex=false, width=1.05\columnwidth]{figs/figures-ThematicEquivalenceDef.drawio.svg}
    \caption{}
    \label{fig:thematic_equiv_def}
    % \vspace{-0.4cm}
\end{figure}



Thematic theory \cite{} is one of the most popular representations of sentence semantics.
The theory abstracts the sentence semantics as the semantic relationship between an event and its participants.
Using the example of Figure~\ref{fig:thematic_equiv_def}, the event is the action of \textit{eat} and the participants are \textit{John} (the actor of the event), \textit{an apple} (the patient of the event), and \textit{this morning} (the time of the event).
The three thematic relations represent the event that the sentence conveys.
% <the relationship with syntax>
The thematic theory is no stranger to linguistic studies.
The theory allows linguists to incorporate and control semantic factors in generative grammar \cite{}.

% The two sentences describe the same event but have different focuses.
% The former is a simple statement of the past event while the latter focuses on the state that the apple has already been eaten.
% Thematic equivalence also differs from the notion of textual entailment, as illustrated by sentences 1 and 3 in Figure \ref{}.
% Sentence 1 entails sentence 3 in that sentence 1 has additional information about the time of the event.
% However, they are not thematically equivalent because the time \textit{this morning} is also a participant in the event.

% <allowing missing evidence> will result in the reduction of evidence.

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
    \adjustbox{max width=\columnwidth}{
        % \small
        \begin{tabular}{|l|l|}
            \hline
            Treebank   & Results were released after the market closed.           \\
                       & Options markets stopped trading in many securities.      \\
                       & But such spots can be too soft.                          \\
                       & Mr. Bandow is a Cato Institute fellow.                   \\\hline
            Linguistic & the book with a red cover from Blackwell by Robert Burns \\
                       & the book from Blackwell with a red cover by Robert Burns \\
                       & the book from Blackwell by Robert Burns with a red cover \\
                       & the book by Robert Burns from Blackwell with a red cover \\\hline
        \end{tabular}
    }
    \caption{A comparison of data in Penn Treebank and data used in linguistic study. The linguistic data is taken from \citet{Carnie2007-CARSAG} in the discussion of adjuncts.}
    \label{tbl:treebank_vs_linguistics}

\end{table}

Previous unsupervised constituency parsing research focused on either inducing a large and complex grammar from a natural language corpus \cite{} or measuring how well a span can stand alone as a constituent with language models \cite{}.
Both methods operate upon a dataset containing sentences with diverse semantics and syntactic structures, as shown in the first part of Table~\ref{tbl:treebank_vs_linguistics}.
The word-sequence pattern in such a dataset can be attributed to both syntactic and semantic factors.
In contrast, linguistic studies employ data \cite{Carnie2007-CARSAG} with much better regularity, as shown in the second part of Table~\ref{tbl:treebank_vs_linguistics}.
The three sentences, despite being textually different, share the same thematic relations.
As a result, linguists can isolate the syntactic factors that result in the word-sequence pattern from the semantic factors.


In this study, we propose to discover the phrase structure by detecting frequent word-sequence patterns among thematically equivalent sentences.
We refer to two sentences as thematically equivalent when the two sentences have the same thematic relations (i.e., describing the same event with the same set of participants).
Sentences 1 and 2 in Figure \ref{fig:thematic_equiv_def} form a thematic equivalence class, but they are not semantically identical.
Sentence 1 is a simple statement of the past event while sentence 2 focuses on the state of the apple.
Sentences 1 and 3 do not form a thematically equivalence class because sentence 1 contains additional information about the time of the event.
Consequently, Sentence 1 and 3 are not thematically equivalent.

\begin{figure}[t]
    \centering
    \includesvg[inkscapelatex=false, width=0.8\columnwidth]{figs/figures-Target'nThematicEquivalentExamples.drawio.svg}
    \caption{A target sentence and a set of generated sentences that is thematically equivalent to the target sentence. We highlight participants that are common in the thematic equivalence class in bold.}
    \label{fig:thematic_equiv_example}
    % \vspace{-0.4cm}
\end{figure}

Figure~\ref{fig:thematic_equiv_example} illustrates a target sentence that we want to parse and a set of generated sentences that are in the same thematic equivalence class as the target sentence.
We have two observations: (1) word sequences denoting the participants frequently occur in the equivalent sentences; (2) word sequences denoting the event occur less frequently than the word sequence denoting the participants.
We hypothesize that \textbf{constituents are frequent word-sequence patterns among thematically equivalent sentences, although the frequency may vary between constituent types}.

We propose a span-overlap score that measures the word sequence frequency among thematically equivalent sentences, in order to verify and apply the hypothesis in unsupervised constituency parsing.
Given a target sentence that we want to parse, we gather the thematically equivalent sentence from an instruction following language model (e.g., \texttt{ChatGPT}) using 4 types of theme-preserving instructions.
We match each word sequence in the target sentence against the equivalent sentence and measure the word sequence frequency.
By our hypothesis, word sequences with higher invariability would have a higher chance of occurring in the equivalent sentences (i.e., higher occurrence frequency).
We treat the occurrence frequency as the span score and perform parsing by decoding a tree with a maximum total span score.
We analyze the span score for each constituent type across multiple languages.

The contributions of this study are 4 fold:
(1) A novel, multilingually applicable, and state of the art unsupervised constituency parser that discovers the phrase structure based on surface word sequence statistics.
(2) Empirically showing that constituents denoting participants in an event occur more frequently than constituents denoting the event.
(3) Showcasing the qualitative difference in the invariability between the participant-related constituents and event-related constituents across multiple languages.
(4) Indicating the importance of thematic relations in the task of unsupervised constituency parsing.
% \end{itemize}
